Synthesizing the Optimal Luenberger-type Observer for Nonlinear Systems

Observer design typically requires the observability of the underlying system, which may be hard to verify for nonlinear systems, while guaranteeing asymptotic convergence of errors, which may be insufficient in order to satisfy performance conditions in finite time. This paper develops a method to design Luenberger-type observers for nonlinear systems which guarantee the largest possible domain of attraction for the state estimation error regardless of the initialization of the system. The observer design procedure is posed as a two step problem. In the the first step, the error dynamics are abstractly represented as a linear equation on the space of Radon measures. Thereafter, the problem of identifying the largest set of initial errors that can be driven to within the user-specified error target set in finite-time for all possible initial states, and the corresponding observer gains, is formulated as an infinite-dimensional linear program on measures. This optimization problem is solved, using Lasserre's relaxations via a sequence of semidefinite programs with vanishing conservatism. By post-processing the solution of step one, the set of gains that maximize the size of tolerable initial errors is identified in step two. To demonstrate the feasibility of the presented approach two examples are presented.

==> arxiv/sections/abstract.tex <==
\begin{abstract}
	Accurately modeling and verifying the correct operation of systems interacting in dynamic environments is challenging.
	By leveraging parametric uncertainty within the model description, one can relax the requirement to describe exactly the interactions with the environment; however, one must still guarantee that the model, despite uncertainty, behaves acceptably. 
	This paper presents a convex optimization method to efficiently compute the set of configurations of a polynomial dynamical system that are able to safely reach a user defined target set despite parametric uncertainty in the model.
	Since planning in the presence of uncertainty can lead to undesirable conservativeness, this paper computes those trajectories of the uncertain nonlinear systems which are $\alpha$-probable of reaching the desired configuration.
	The presented approach uses the notion of occupation measures to describe the evolution of trajectories of a nonlinear system with parametric uncertainty as a linear equation over measures whose supports coincide with the trajectories under investigation.
	This linear equation is approximated with vanishing conservatism using a hierarchy of semidefinite programs each of which is proven to compute an approximation to the set of initial conditions that are $\alpha$-probable of reaching the user defined target set safely in spite of uncertainty.
	The efficacy of this method is illustrated on four systems with parametric uncertainty.
\end{abstract}

==> arxiv/sections/conc.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this paper, a convex optimization technique to approximate the $\alpha$-confidence backwards reachable set of a parametrically uncertain system is presented. Using the notion of occupation measures, we propose a two step methodology to construct a sequence of convergent approximations of the set of interest -- the first step optimizes over the space of the ring of polynomials with a specified degree and is solved as a sums-of-square program; the second step builds on the result of the first step and constructs an outer approximation of the $\alpha$-confidence reachable set. The proposed method is validated numerically on three examples of varying complexities.


==> arxiv/sections/implementation.tex <==
\section{Numerical Implementation}
\label{sec:implementation}

In this section, a sequence of Semidefinite Programs (SDPs) that approximate the solution to the infinite dimensional primal and dual defined in Sec.~\ref{sec:prob} are introduced.

\subsection{Lasserre's relaxations}
This sequence of relaxations is constructed by characterizing each measure using a sequence of moments\footnote{The $n$th moment of a measure ($\mu$) is obtained by evaluating the following expression
  $$y_{\mu,n}=\ip{\mu,x^n}.$$}
and assuming the following:
\begin{assum}
The dynamical system in Eqn. \eqref{eq:aug_system} is a polynomial.
Moreover the domain, the set of possible values of uncertainties, and the target set are semi-algebraic sets.
  \label{assump:poly}
\end{assum}
Recall that polynomials are dense in the set of continuous functions by the Stone-Weierstrass Theorem so this assumption is made without too much loss of generality.
\par
Under this assumption, given any finite $d$-degree truncation of the moment sequence of all measures in the primal $(P)$, a primal relaxation, $(P_d)$, can be formulated over the moments of measures to construct an SDP.
The dual to $(P_d)$, $(D_d)$, can be expressed as a sums-of-squares (SOS) program by considering $d$-degree polynomials in place of the continuous variables in $D$.
\par
To formalize this dual program, first note that a polynomial $p \in \R[x]$ is SOS or $p \in \text{SOS}$ if it can be written as $p(x) = \sum_{i=1}^m q_i^2(x)$ for a set of polynomials $\{q_i\}_{i=1}^m \subset \R[x]$.
Note that efficient tools exist to check whether a finite dimensional polynomial is SOS using SDPs~\cite{parrilo2000structured}.
Next, suppose we are given a semi-algebraic set $A = \{x \in \R^n \mid h_{i}(x) \geq 0, h_i \in \R[x], \forall i \in \N_m \}$.
We define the $d$-degree {\em quadratic module} of $A$ as:
\begin{align}
  \begin{split}
  Q_d(A)=\bigg\{q\in \R_d[x]\,\bigg|\, \exists \{s_k\}_{k \in \{0,1,...,m\} \cup \{0\}} \subset \text{SOS s.t. } \\
  q=s_0+\sum_{k\in \{1,...,m\}}h_{k}s_k \bigg\}
  \end{split}
\end{align}

\noindent The $d$-degree relaxation of the dual, $D_d$, can now be written as:
  \begin{flalign}\nonumber
    & & \inf_{\Xi_d} \hspace*{0.1cm} & \int_{X\times \Theta}w_d(x,\theta)\,d(\lambda_x\otimes\lambda_\theta) && \hspace*{-0.3cm} (D_d) \nonumber\\
    & & \text{st.} \hspace*{0.1cm} & w_d\in Q_d(X\times \Theta) && \\
    & & & v_d(T,x,\theta)\in Q_d(X_T \times \Theta) && \\
    & & & -\mathcal L_{f}v_d(t,x,\theta)\in Q_d(\mathcal T\times X \times \Theta) && \\
    & & & w_d-v_d(0,x,\theta)-1\in Q_d(X\times \Theta)
  \end{flalign}
where $\Xi_d=\Big\{ \big(v_d,w_d\big) \in \R_d[t,x,\theta]\times \R_d[x,\theta]\Big\}$.
A primal can similarly be constructed, but the solution to the dual can be used to directly generate a sequence of outer approximations to the uncertain backwards reachable set:
\begin{lem}
Let $w_d$ denote the $w$-component of the solution to $(D_d)$. Then $X_{(0,d)} = \{(x,\theta) \in X\times \Theta \mid w_d(x,\theta) \geq 1 \}$ is an outer approximation to $\spt(\mu_0)$ and $\lim_{d\to\infty}\lambda_x\otimes \lambda_\theta({ X}_{(0,d)} \backslash \spt(\mu_0)) = 0$.
\end{lem}
Using the finite-degree truncation of the infinite dimensional problem presented above, one can solve for a sequence of convergent approximations of the support of $\mu_0$. To approximate the BRS as defined in Defn.~\ref{defn:brs}, we need to perform an additional step, described in the next section.

\subsection{Generating outer approximations of $X_0^\alpha$}
This section presents two methods to use the outer approximations of $\spt(\mu_0)$ derived by solving $(D_d)$, to estimate $X_0^\alpha$ as defined in Defn.~\ref{defn:brs}. The first method relies on discretizing the state space and computing the probability that each node in the mesh will reach the target set $X_T$ at $t=T$, through Monte Carlo simulation. The second method poses an additional optimization problem over polynomial functions that computes a polynomial representation to the level sets of interest. This second formulation can be solved by using semidefinite programming.
\subsubsection{A direct numerical approach}
\label{sssec:direct}
Given a value of $x$, to compute the probability of success, discretize the space of uncertainty, compute the spread of the $w_d$ that solves $(D_d)$ with respect to $\theta$ as the following
 \begin{align}
   \beta :=\sum_{i=1}^N \min(1,w(x,\theta_i))^k f_\theta(\theta_i)
   \label{eq:beta}
 \end{align}
 where $k\ge 1$, $\{\theta_i,\forall i\in \{1,\ldots,N\}\}$ is the set of discrete values of $\theta$, and $f_\theta(\theta)$ is the density (converted appropriately to a probability mass function) of $\mu_\theta$ with respect to $\lambda_\theta$.
\subsubsection{A more generic method}
Consider the following optimization problem for a given value of $k$
\begin{flalign}
  &&\sup_{q,r} & \phantom{3}\ip{\lambda\otimes \mu_\theta,q} +\ip{\mu_\theta,r} && (PP)\\
  &&\text{st. }&\phantom{3} 0\le q(x,\theta)\le 1                               && \forall (x,\theta)\in X\times \Theta\\
  &&& \phantom{3} q(x,\theta) \le w(x,\theta)^k                                 && \forall (x,\theta)\in X\times \Theta\\
  &&& \phantom{3}0\le r(x)\le \ip{\mu_\theta,q}                                 && \forall x\in X\\
  &&& \phantom{3}r\in \R[x]\\
  &&& \phantom{3}q\in \R[x,\theta]
\end{flalign}
The function $r$ is the function that traces the probability that every $x$ can reach $X_T$.


==> arxiv/sections/introduction.tex <==
\section{Introduction}

Verifying the correct operation of systems interacting in dynamic environments is challenging.
In fact, the difficulties associated with modeling such systems exactly compounds this verification challenge.
By introducing parametric uncertainty within the model, one can compensate directly for the inability to construct exact models; however, to ensure the satisfactory operation of uncertain systems one must provide systematic guarantees on all probable behaviors.
Unfortunately, unforeseen conservativeness may arise when certain low probability outcomes restrict the potential behavior of the system.
To address this shortcoming, this paper presents an approach to compute the set of initial conditions of a nonlinear system with parametric uncertainty that are at least $\alpha$-probable of arriving at a user defined target set. 

% talk about barrier certificates
A variety of numerical methods have been proposed to verify the satisfactory operation of nonlinear systems with parametric uncertainty. 
The most popular of these approaches have relied upon generating or evaluating pre-constructed Lyapunov functions to compute the domain of attraction of an uncertain system \cite{chesi2004estimating,topcu2007stability}.
This has required checking Lyapunov's criteria for polynomial systems by using sums-of-squares programming, which results in a bilinear optimization problem that is usually solved using some form of alternation \cite{prajna2007convex}. 
However, such methods are not guaranteed to converge to global optima (or necessarily even local optima), and require feasible initializations.

Others have developed tools to perform safety verification of more general stochastic nonlinear dynamical systems \cite{mitchell2005time,prajna2007framework}. 
Hamilton-Jacobi Bellman based approaches, for example, have also been applied to compute the uncertain backwards reachable set for nonlinear systems with arbitrary uncertainty affecting the state at any instance in time \cite{mitchell2005time}.
These approaches solve a more general problem and scale well despite state space discretization when the specific system under consideration has special structure \cite{maidens2013lagrangian}.
Barrier certificate methods \cite{prajna2007convex} have also been utilized to perform stochastic safety verification by using a super martingale. 

% speak about occupation measure approach/our method
This paper leverages a method developed in a recent paper that describes the evolution of trajectories of an uncertain dynamical system using a linear equation over measures \cite{mohan2016convex}. 
As a result of this characterization, the set of configurations that are able to reach a target set despite parametric uncertainty, called the \emph{uncertain backwards reachable set}, can be computed as the solution to an infinite dimensional linear program over the space of nonnegative measures.
This approach, which was inspired by several recent papers \cite{henrion2014convex,majumdar2014convex,shia2014convex}, computes an approximate solution to this infinite dimensional linear program using a sequence of finite dimensional relaxed semi-definite programs via Lasserre's hierarchy of relaxations \cite{lasserre2001global} that each satisfy an important property:
each solution to this sequence of semi-definite programs is an outer approximation to the uncertain backwards reachable set with asymptotically vanishing conservatism.
Our approach will utilize this same formulation to construct an outer approximation to the set of $\alpha$-probable points in the uncertain backwards reachable set which we call the \emph{$\alpha$-level backwards reachable set}.

% talk about the paper by sloth
This approach of characterizing the behavior of the system using an infinite dimensional program over measures has also been used to perform safety verification of stochastic nonlinear systems \cite{sloth2015safety}. 
In that instance, initial conditions of the stochastic system whose trajectories on \emph{average}
have probability higher than some user-specified $p$ of arriving at some target set were computed using a semidefinite programming hierarchy.
In this paper, we consider instead the problem of determining which set of initial conditions of a dynamical system have a user-specified probability of arriving at a target set under parametric uncertainty within the model. 
Since there is no stochastic behavior in the dynamical system, our approach does not consider an average probability over each trajectory.


% summarize our paper
The remainder of the paper is organized as follows:
Section \ref{sec:preliminaries} introduces the notation used in the remainder of the paper, the class of systems under consideration, and the backwards reachable set problem under parametric uncertainty;
Section \ref{sec:prob} describes how the $\alpha$-level backwards reachable set under parametric uncertainty is the solution to an infinite dimensional linear program;
Section \ref{sec:implementation} constructs a sequence of finite dimensional semidefinite programs that outer approximate the infinite dimensional linear program with vanishing conservatism;
Section \ref{sec:examples} describes the performance of the approach with three examples;
and, Section \ref{sec:conclusion} concludes the paper.



==> arxiv/sections/prelim.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

This section describes the class of systems under consideration and outlines the problem of interest.
\subsection{Notation}
In the remainder of this text the following notation is adopted: sets are italicized and capitalized (ex. $K$). The set of continuous functions on a compact set $K$ are denoted by $\mathcal C(K)$.
The ring of polynomials in $x$ is denoted by $\R[x]$, and the degree of a polynomial is equal to the degree of its largest multinomial; the degree of the multinomial $x^\alpha,\,\alpha\in \N_{\ge 0}^n$ is $|\alpha|=\|\alpha\|_1$; and $\R_d[x]$ is the set of polynomials in $x$ with maximum degree $d$.
The dual to $\mathcal C(K)$ is the set of Radon measures on $K$, denoted as $\mathcal M(K)$, and the pairing of $\mu\in \mathcal M(K)$ and $v\in \mathcal C(K)$ is:
  \begin{align}
  \ip{\mu,v}=\int_{K}v(x)\,d\mu(x).
  \end{align}
We denote the nonnegative Radon measures by ${\cal M}_+(K)$. The space of Radon probability measures on $K$ is denoted by ${\cal P}(K)$.
The Lebesgue measure is denoted by $\lambda$. Finally, the support of measures, $\mu$, is identified as $spt(\mu)$.
\subsection{System class}
In this paper, we restrict our attention to the class of parametrically uncertain drift systems; i.e. systems of the following form:
\begin{align}
  \dot {x} = f(x,\theta),
\end{align}
where $x\in X$, are the states of the system, and $\theta\in \Theta$ are uncertain parameters.
\begin{assum}
  $X$ and $\Theta$ are compact, and $f$ is Lipschitz continuous in $x$ and $\theta$.
\end{assum}
\begin{ex}[Van der Pol Oscillator]
Consider the uncertain Van der Pol oscillator whose dynamics is:
  \begin{align}
  \begin{aligned}
  \dot x_1 =&\,    -2x_2\\
  \dot x_2=&\,    0.8x_1+(9+5\theta)x_2(x_1^2-0.21)
    \end{aligned}
\end{align}
where $\theta \in [-0.5,0.5]$ and $x(t)\in X=[-1,1]$. In this example, the limit cycle of the Van der Pol oscillator deforms as the value of $\theta$ changes: the larger the value of $\theta$, the smaller the volume of the area contained inside the limit cycle.
\end{ex}
Parameters $\theta\in \Theta$ are assumed to be drawn according to a probability distribution $\mu_\theta\in \mathcal P(\Theta)$.
\begin{assum}
  If the uncertain parameter $\theta$ is distributed according to $\mu_\theta$, $\mu_\theta$ is absolutely continuous with respect to the Lebesgue measure. We denote this by: $\mu_\theta \ll \lambda_\theta$, where $\lambda_\theta$ is the Lebesgue measure on $\spt(\mu_\theta)$.
\end{assum}
It is assumed that the unknown parameters do not change with time and that they are instantiated at time $t=0$. That is, the uncertain system can be thought to evolve in the embedded space $X\times \Theta$ according to the following dynamics
\begin{align}
    \begin{bmatrix}
    \dot {x}\\\dot \theta
  \end{bmatrix} = \begin{bmatrix}
    f(x,\theta)\\0
  \end{bmatrix}.
  \label{eq:aug_system}
\end{align}
For notational convenience, we denote the unique solution to the dynamics in Eqn.~(\ref{eq:aug_system}) as the absolutely continuous function $\gamma$ defined as follows:
\begin{align}
  \gamma : [0,T]\xrightarrow{\text{Eqn.}~(\ref{eq:aug_system})} X\times \Theta,\phantom{3} \gamma(0) = [x;\theta].
\end{align}
In addition, let us denote by $\mathcal T$, the time interval $[0,T]$.
\subsection{Problem Description}
The objective of this paper is to identify the $\alpha$-confidence, time limited reachable set, or \emph{uncertain backwards reachable set} (BRS) of $X_T$. This definition relies on the following set-valued mapping from $X$ to the Borel $\sigma$-algebra on $\Theta$ (closed sets), $\mathcal B(\Theta)$:
\begin{align}
\begin{split}
  \Gamma(x)=\{\theta \in \Theta\mid \exists\, \gamma :\mathcal T\xrightarrow{\text{Eqn.}~(\ref{eq:aug_system})} X\times \Theta, \text{ with }\\
  \gamma(0)= [ x ;\theta],\gamma(T)\in X_T\times \Theta\}.
\end{split}
\label{eq:Gamma}
\end{align}
For a given value of $x\in X$, $\Gamma(x)$ is the set of distinct values of the parameter $\theta$, such that the solution trajectories of the system in Eqn.~(\ref{eq:aug_system}), with the states initialized to $[x;\Gamma(x)]$ arrives at $X_T$ at time $T$.
\begin{defn}
\label{defn:brs}
  The $T$-time $\alpha$-confidence backwards reachable set of $X_T$, under the dynamics in Eqn.~(\ref{eq:aug_system}), is the defined as follows
  \begin{align}
    X_0^{\alpha} = \{x_0\mid \mu_\theta(\Gamma(x_0))\ge \alpha\}
  \end{align}
\end{defn}
The $\alpha$-confidence BRS is the set of initial values of $x$ such that for each $x$, the {\em mass} of $\Gamma(x)$ under $\mu_\theta$ is larger than $\alpha$; i.e. the set of initial conditions for which the probability of arriving in $X_T$ at $t=T$ is greater or equal to $\alpha$.
The remainder of this paper is devoted to tractably computing $X_0^{\alpha}$.


==> arxiv/sections/prob.tex <==
\section{Problem formulation}
\label{sec:prob}
In this section, we present a methodology to compute the time limited $\alpha$-confidence backwards reachable set of dynamic systems. The proposed methodology consists of two steps: (1) estimating the set of all feasible initial conditions of the system in Eqn.~(\ref{eq:aug_system}) such that $\gamma(T)\in X_T\times \Theta$; (2) determining the subset of initial conditions that reach the target set with desired probability. Step (1) is addressed by solving an infinite dimensional problem, and step (2) requires integrating the optimal solution of step (1).

To estimate the BRS, we use the notion of {\em occupation measures} \cite{pitman1977}. Given an initial condition for the system, the occupation measure evaluates to the amount of time spent by the resultant trajectory in any subset of the space. The occupation measure $\mu(\cdot\mid x_0,\theta)\in \mathcal M_+(\mathcal T\times X\times \Theta\mid x_0,\theta)$ is formally defined as follows:
\begin{align}
  \mu(A\times B\times C\mid x_0,\theta) = \int_{0}^T I_{A\times B\times C}(t,x,\theta\mid x_0,\theta)\,dt,
  \label{eq:occ}
\end{align}
where $I_{A}(x)$ is the indicator function on the set $A$ that returns one if $x\in A$ and zero otherwise. With the above definition of the occupation measure, using elementary functions, it can be shown that:
\begin{align}
  \ip{\mu(\cdot\mid x_0,\theta),v} = \ip{\lambda_t,v(t,x(t\mid x_0,\theta),\theta)},
  \label{eq:ip}
\end{align}
where $\lambda_t$ is the Lebesgue measure on $\mathcal T$.

The {\em occupation measure} has an interesting characteristic -- it completely characterizes the solution trajectory of the system resulting from an initial condition. Observe that the occupation measure as defined in Eqn.~(\ref{eq:occ}) is conditioned on the initial values of states and parameters. Since we are interested in the collective behavior of a set of initial conditions, we define the {\em average} occupation measure as:
\begin{align}
\mu(A\times B\times C) = \int_{X\times \Theta} \mu(A\times B\times C\mid x,\theta)\,d\mu_0,
\end{align}
where $\mu_0$ is the un-normalized distribution of initial conditions. The value to which the {\em average} occupation measure evaluates over a given set in $\mathcal T\times X\times \Theta$ can be interpreted as the cumulative time spent by all solution trajectories which begin in $\spt(\mu_0)$.
\par
Given a test function $v\in \mathcal C^1(\mathcal T\times X\times \Theta)$, using the Fundamental Theorem of Calculus, its value at time $t=T$ is given by
\begin{align}
\begin{split}
  v(T,x(T\mid x_0,\theta),\theta) =&\, v(0,x_0,\theta)\\
  +&\,\int\limits_{0}^T\hspace*{-.08in}\left(\frac{\partial v}{\partial x}\cdot f+\frac{\partial v}{\partial t}\right)(t,x(t\mid x_0,\theta),\theta)\,dt
\end{split}
  \label{eq:ftc}
\end{align}
Using the relation defined in Eqn.~(\ref{eq:ip}) and by defining the linear operator $\mathcal L_f$ on $\mathcal C^1$ functions (Lie derivative) as the following:
\begin{align}
  \mathcal L_{f}v = \frac{\partial v}{\partial x}\cdot f+ \frac{\partial v}{\partial t},
\end{align}
Eqn.~(\ref{eq:ftc}) is re-written as
\begin{align}
\begin{split}
  v(T,x(T\mid x_0,\theta),\theta) =&\, v(0,x_0,\theta)\\
  +&\,\int\limits_{X\times \Theta}\mathcal L_{f}v\,d\mu(t,x,\theta\mid x_0,\theta).
\end{split}
\label{eq:ftc2}
\end{align}
Integrating Eqn.~(\ref{eq:ftc2}) with respect to $\mu_0$, the distribution of initial conditions, and defining a new measure $\mu_T\in \mathcal M_+ (X_T\times \Theta)$, as the following
\begin{align}
  \mu_T(A\times B) = \int\limits_{X\times \Theta}I_{A\times B}(x(T\mid x_0,\theta),\theta)\,d\mu_0,
\end{align}
produces the following equality
\begin{align}
  \ip{\delta_T\otimes \mu_T,v}= \ip{\delta_0\otimes \mu_0,v}+\ip{\mu,\mathcal L_{\tilde f}v},
  \label{eq:lv}
\end{align}
where, with a slight abuse of notations, $\delta_t$ is used to denote a Dirac measure situated at time $t$. Using adjoint notations, Eqn.~(\ref{eq:lv}) can be written as:
\begin{align}
  \delta_T\otimes \mu_T= \delta_0\otimes \mu_0+\mathcal L_{f}'\mu
  \label{eq:adjointlv}
\end{align}
Equation~(\ref{eq:adjointlv}) is a version of the Liouville equation, holds for all test function $v\in \mathcal C^1(\mathcal T\times X\times \Theta)$, and summarises the visitation information of all trajectories that emanate from $\spt(\mu_0)$ and terminate in $\spt(\mu_T)$. Several recent papers provide a more detailed discussion on the Liouville equation \cite{henrion2014convex},\cite{mohan2016convex}.
\par
Within this framework of measures and the Liouville Equation, we first formulate the problem of identifying the set of all pairs $(x_0,\theta)$ such that the solution trajectory of the system in Eqn.~(\ref{eq:aug_system}) initialized at $[x;\,\theta]$ arrives at $X_T\times \Theta$ at $t=T$. This problem can be interpreted as one that attempts to identify the largest support for $\mu_0$ that ensures the existence of measures $\mu$ and $\mu_T$ such that $(\mu_0,\mu_T,\mu)$ satisfy Eqn.~(\ref{eq:lv}). To measure the size of $\spt(\mu_0)$, we use the Lebesgue measure on $X\times \Theta$, $\lambda_x\otimes \lambda_\theta$.
\par
This problem is posed as an infinite dimensional Linear Program (LP) on measures as defined below.
%
%To identify the $\alpha$-confidence
%
%can be formulated as the following infinite-dimensional linear program that supremizes the \emph{volume} of the set of initial pairs of $x$ and uncertain parameter, $\theta$, such that the state trajectories, at time $T$, arrive in $X_T$ :
\begin{flalign}\nonumber
    & & \sup_{\Lambda} \hspace*{1cm} & \ip{\mu_{0},\mathds 1} && (P)\\
    & & \text{st.} \hspace*{1cm} &\mu_{0}+\mathcal L_{f}'\mu=\,\mu_{T} && \label{eq:primal:liouville}\\
    & & & \mu_{0}+\hat\mu_{0}=\,\lambda_x\otimes \lambda_\theta &&
\end{flalign}
where $\lambda_x\otimes \lambda_\theta$ is the Lebesgue measure supported on $X\times \Theta$, $\Lambda:=(\mu_0,\hat\mu_{0},\mu_T) \in {\mathcal M}_+({\mathcal T} \times X \times \Theta) \times \mathcal M_+( X \times \Theta)\times \mathcal M_+( X_{T}\times \Theta )$ and $\mathds 1$ denotes the function that takes value $1$ everywhere.
\begin{lem}
  The support of $\mu_0$, $\spt(\mu_0)\subset X\times \Theta$ is the largest collection of pairs $(x,\theta)$ that, if used as initial conditions to Eqn. \eqref{eq:aug_system}, produce a solution trajectory that terminates in $X_T\times \Theta$ at $t=T$.
\end{lem}
\par
The dual problem, on continuous functions, corresponding to $(P)$ is the following
\begin{flalign}\nonumber
  & &  \inf_{\Xi}&\phantom{3} \ip{\lambda_x\otimes \lambda_\theta,w}          && (D) \nonumber \\
  & &  \text{st.}&\phantom{3}\mathcal L_{f} v(t,x,\theta)\le 0         && \forall (t,x,\theta)\in \mathcal T\times X\times\Theta\\
  & &  &\phantom{3} w(x,\theta) \ge 0                                         && \forall (x,\theta)\in X\times\Theta\\
  & &  &\phantom{3} w(x,\theta) - v(0,x,\theta) - 1 \ge 0                     && \forall (x,\theta)\in X\times\Theta\\
  & & & \phantom{3} v(T,x,\theta)\ge 0                                        && \forall (x,\theta)\in X_T\times \Theta
\end{flalign}
where $\Xi := (v,w)\in \mathcal C^1(\mathcal T\times X\times \Theta)\times \mathcal C(X\times \Theta)$. The solution to $(D)$ has an interesting interpretation: $v$ is similar to a Lyapunov function for the system, and $w$ resembles an indicator function on $\spt(\mu_0)$. Moreover:
\begin{lem}
  There is no duality gap between problems $(P)$ and $(D)$.
\end{lem}
\begin{lem}
  Given the pair of functions $(v^*,w^*)$ which is the optimal solution to $(D)$, the 1-super-level set of $w^*$ contains $\spt(\mu_0)$.
\end{lem}
The following salient result on the shape of $w$ is the critical result that we will employ to estimate $X_0$ as defined in Defn.~\ref{defn:brs}.
\begin{thm}\cite[Theorem~3]{henrion2014convex}
\label{thm:indicator}
 There is a sequence of feasible points to $(D)$ whose $w$ component converges uniformly in the $L^1$ norm to the indicator function on $\spt(\mu_0)$.
\end{thm}
An immediate consequence of the above theorem is that we can assume that $w$ evaluates to one on $\spt(\mu_0)$ and zero elsewhere. Now, relating the definition of $\Gamma$ in Eqn.~(\ref{eq:Gamma}) and this feature of $w^*$, the $w$-component of the optimal solution of $(D)$, one arrives at the following result that provides a means to compute the $\alpha$-confidence time limited reachable set, $X_0^\alpha$.
\begin{lem}
Suppose $(v^*,w^*)$ is an optimal solution of $(D)$. The $\alpha$-level backwards reachable of the set $X_T$ under the system dynamics of Eqn. (4) and parametric uncertainty with distribution $\mu_\theta$ is given by the following set
\begin{align}
X_0^\alpha:=\bigg\{x\,\big \mid \int_\Theta w^*(x,\theta)\,d\mu_\theta\ge \alpha \bigg\}
\end{align}
\label{lem:confidence}
\end{lem}
\begin{proof}
%There exists a sequence $w_k$ of feasible $w$ in $(D)$ that converges to the indicator function $I_{\Gamma(x)}(x,\theta)$ in the $L^1$ norm (REFERENCE H-K PAPER). Therefore, the optimal solution $w^*$ is $I_{\Gamma(x)}(x,\theta)$. So, for any $x$,
%\begin{align}
%\int_\Theta w^*(x,\theta)\,d\mu_\theta &= \int_{\Gamma(x)} \mathds 1\,d\mu_\theta = \mu_\theta(\Gamma(x))
%\end{align}
Using the provided information, define the measure $\eta\in \mathcal M_+(X\times \Theta)$ as follows:
\begin{align}
  \eta(A\times B) = \int_{A\times B} w^*(x,\theta) \,d(\lambda_x\otimes \mu_\theta).
\end{align}
It should be noted that $\Gamma(x)$ as defined in Eqn.~(\ref{eq:Gamma}) is the support of the conditional distribution of $\theta$ given $x$ of $\eta$; $\spt(\eta(\cdot\mid x))$. This is true since $w^*$ is an indicator function on $\spt(\mu_0)$, the set of all feasible pairs $(x,\theta)$.
In addition, by definition, $\lambda_x\otimes \mu_\theta \gg \eta$ and hence $\lambda_x\gg \pi^x_*\eta$, where $\pi^x_*\eta$ is the push-forward measure of $\eta$ under the $x$-projection operation as per \cite{lee2003smooth}. Thus, $\phi(x)$, $\lambda_x$ measurable, is the Radon-Nikodym derivative between $\lambda_x$ and $\pi_*^{x}\eta$ such that
\begin{align}
  \pi^x_*\eta(A) =&\, \int_A \phi(x)\,d\lambda_x,\phantom{4}\forall A\subset X.
\end{align}
The function $\phi(x)$, for each $x$ evaluates to the probability that $x$ will reach $X_T$ given the distribution of uncertainty. To see this, observe that
\begin{align}
  \int_A \phi(x)\,d\lambda_x = &\,\int_A \int_\Theta w^*\,d\,\mu_\theta d\lambda_x,\\
  =&\, \int_A \int_{\Gamma(x)} w^*\,d\,\mu_\theta d\lambda_x,\\
  =&\, \int_A \int_{\Gamma(x)} 1\,d\,\mu_\theta d\lambda_x,
\end{align}
where we have used the fact that $w^*\ge 1,\, \forall(x,\theta)\in \spt(\mu_0)$ (from Thm.~\ref{thm:indicator}), that $\mu_\theta$ is a probability measure, and Defn.~\ref{defn:brs}. The statement of the Lemma now follows from Defn.~\ref{defn:brs}.
\end{proof}
Lemma~\ref{lem:confidence} provides a means to compute the $\alpha$-confidence $T$-time backwards reachable set; one just has to integrate the $w$ component of the optimal solution to $(D)$ with respect to the distribution of $\theta$ and identify level sets. Solving the infinite dimensional problem is nontrivial; in the following section, we employ Lasserre's hierarchy of relaxations to arrive at a sequence of outer approximations of $X_0^\alpha$.


==> arxiv/sections/prob_conf.tex <==
\section{Problem formulation}
\label{sec:prob}
<<<<<<< .mine
In this section, we present a methodology to estimate the time limited $\alpha$-confidence backwards reachable set of dynamic systems. The proposed methodology consists of two steps -- (1) estimating the set of all feasible initial conditions of the system in Eqn.~(\ref{eq:aug_system}) such that $\gamma(T)\in X_T\times \Theta$; (2) determining the subset of initial conditions that reach the target set with desired probability. The first step is addressed by solving one of a pair of infinite dimensional problems, and the second step is performed on the optimal solution of Step (1).
\par
To estimate the BRS, we use the notion of {\em occupation measures} which was first introduced in \cite{Pitman1977}. Given an initial condition for the system, the occupation measure evaluates to the amount of time spent by the resultant trajectory in any subset of the space. The occupation measure $\mu(\cdot\mid x_0,\theta)\in \mathcal M_+(\mathcal T\times X\times \Theta\mid x_0,\theta)$ is formally defined as follows:
=======
In this section, we present a methodology to compute the time limited $\alpha$-confidence backwards reachable set of dynamic systems. The proposed methodology consists of two steps -- (1) estimating the set of all feasible initial conditions of the system in Eqn.~(\ref{eq:aug_system}) such that $\gamma(T)\in X_T\times \Theta$; (2) determining the subset of initial conditions that reach the target set with desired probability. The first step is addressed by solving an infinite dimensional problem, and the second step requires integrating the optimal solution of Step (1).

To estimate the BRS, we use the notion of {\em occupation measures} [Pitman]. Given an initial condition for the system, the occupation measure evaluates to the amount of time spent by the resultant trajectory in any subset of the space. The occupation measure $\mu(\cdot\mid x_0,\theta)\in \mathcal M_+(\mathcal T\times X\times \Theta\mid x_0,\theta)$ is formally defined as follows:
>>>>>>> .r67
\begin{align}
  \mu(A\times B\times C\mid x_0,\theta) = \int_{0}^T I_{A\times B\times C}(t,x,\theta\mid x_0,\theta)\,dt,
  \label{eq:occ}
\end{align}
where $I_{A}(\cdot)$ is the indicator function on the set $A$ that returns one if $x\in A$ and zero otherwise. With the above definition of the occupation measure, using elementary functions, it can be shown that:
\begin{align}
  \ip{\mu(\cdot\mid x_0,\theta),v} = \ip{\lambda_t,v(t,x(t\mid x_0,\theta),\theta)},
  \label{eq:ip}
\end{align}
where $\lambda_t$ is the Lebesgue measure on $\mathcal T$.

The {\em occupation measure} has an interesting characteristic -- it completely characterizes the solution trajectory of the system resulting from an initial condition. Observe that the occupation measure as defined in Eqn.~(\ref{eq:occ}) is conditioned on the initial values of states and parameters. Since we are interested in the collective behavior of possibly collection of initial conditions, we define the {\em average} occupation measure as:
\begin{align}
\mu(A\times B\times C) = \int_{X\times \Theta} \mu(A\times B\times C\mid x,\theta)\,d\mu_0,
\end{align}
where $\mu_0$ is the un-normalized distribution of the initial conditions. The value to which the {\em average} occupation measure evaluates over a given set in $\mathcal T\times X\times \Theta$ can be interpreted as the cumulative time spent by all solution trajectories which begin in $\spt(\mu_0)$.
\par
Given a test function $v\in \mathcal C^1(\mathcal T\times X\times \Theta)$, using the Fundamental Theorem of Calculus, its value at time $t=T$ is given by
\begin{align}
\begin{split}
  v(T,x(T\mid x_0,\theta),\theta) =&\, v(0,x_0,\theta)\\
  +&\,\int\limits_{0}^T\hspace*{-.08in}\left(\frac{\partial v}{\partial x}\cdot \tilde f+\frac{\partial v}{\partial t}\right)(t,x(t\mid x_0,\theta),\theta)\,dt
\end{split}
  \label{eq:ftc}
\end{align}
Using the relation defined in Eqn.~(\ref{eq:ip}) and by defining the linear operator $\mathcal L_f$ on $\mathcal C^1$ functions (Lie derivative) as the following:
\begin{align}
  \mathcal L_{\tilde f}v = \frac{\partial v}{\partial x}\cdot \tilde f+ \frac{\partial v}{\partial t},
\end{align}
Eqn.~(\ref{eq:ftc}) is re-written as
\begin{align}
\begin{split}
  v(T,x(T\mid x_0,\theta),\theta) =&\, v(0,x_0,\theta)\\
  +&\,\int\limits_{X\times \Theta}\mathcal L_{\tilde f}v\,d\mu(t,x,\theta\mid x_0,\theta).
\end{split}
\label{eq:ftc2}
\end{align}
Integrating Eqn.~(\ref{eq:ftc2}) with respect to $\mu_0$, the distribution of initial conditions, and defining a new measure $\mu_T\in \mathcal M_+ (X_T\times \Theta)$, as the following
\begin{align}
  \mu_T(A\times B) = \int\limits_{X\times \Theta}I_{A\times B}(x(T\mid x_0,\theta),\theta)\,d\mu_0,
\end{align}
produces the following equality
\begin{align}
  \ip{\delta_T\otimes \mu_T,v}= \ip{\delta_0\otimes \mu_0,v}+\ip{\mu,\mathcal L_{\tilde f}v},
  \label{eq:lv}
\end{align}
<<<<<<< .mine
where with a slight abuse of notations, $\delta_t$ is used to denoted a dirac measure situated at $t$. Equation~(\ref{eq:lv}) is a version of the Liouville equation, holds for all test function $v\in \mathcal C^1(\mathcal T\times X\times \Theta)$, and summarises the visitation information of all trajectories that emanate from $\spt(\mu_0)$ and terminate in $\spt(\mu_T)$. The interested reader to directed to \cite{henrion2014convex} to a more detailed discussion on the Liouivlle equation and the implication of the existence of measures that satisfy the same.
\par
=======
where with a slight abuse of notations, $\delta_t$ is used to denoted a dirac measure situated at $t$. Equation~(\ref{eq:lv}) is a version of the Liouville equation, holds for all test function $v\in \mathcal C^1(\mathcal T\times X\times \Theta)$, and summarises the visitation information of all trajectories that emanate from $\spt(\mu_0)$ and terminate in $\spt(\mu_T)$. Several recent papers provide a more detailed discussion on the Liouville equation [Henrion].

>>>>>>> .r67
Within this framework of measures and the Liouville Equation, we first formulate the problem of identifying the set of all pairs $(x_0,\theta)$ such that the solution trajectory of the system in Eqn.~(\ref{eq:aug_system}) initialized at $[x;\,\theta]$ arrives at $X_T\times \Theta$ at $t=T$. This problem can be interpreted as one that attempts to identify the largest support for $\mu_0$ such that there exist measures $\mu$ and $\mu_T$ such that $(\mu_0,\mu_T,\mu)$ satisfy Eqn.~(\ref{eq:lv}). To measure the size of $\spt(\mu_0)$, we use the Lebesgue measure on $X\times \Theta$, $\lambda_x\otimes \lambda_\theta$.
\par
This problem is posed as an infinite dimensional Linear Program (LP) on measures as defined below.
%
%To identify the $\alpha$-confidence
%
%can be formulated as the following infinite-dimensional linear program that supremizes the \emph{volume} of the set of initial pairs of $x$ and uncertain parameter, $\theta$, such that the state trajectories, at time $T$, arrive in $X_T$ :
\begin{flalign}\nonumber
    & & \sup_{\Lambda} \hspace*{1cm} & \ip{\mu_{0},\mathds 1} && (P)\\
    & & \text{st.} \hspace*{1cm} &\mu_{0}+\mathcal L_{f}'\mu=\,\mu_{T} && \label{eq:primal:liouville}\\
    & & & \mu_{0}+\hat\mu_{0}=\,\lambda_x\otimes \lambda_\theta &&
\end{flalign}
where $\lambda_x\times \lambda_\theta$ is the Lebesgue measure supported on $X\times \Theta$, $\Lambda:=(\mu_0,\hat\mu_{0},\mu_T),\in {\mathcal M}_+({\mathcal T} \times X \times \Theta) \times \mathcal M_+( X \times \Theta)\times \mathcal M_+( X_{T}\times \Theta )$, and $\mathds 1$ denotes the function that takes value $1$ everywhere.
\begin{lem}
  The support of $\mu_0$, $\spt(\mu_0)\subset X\times \Theta$ is the largest collection of pairs $(x,\theta)$ that, if used as initial conditions to Eqn. \eqref{eq:aug_system}, produce a solution trajectory that terminates in $X_T\times \Theta$ at $t=T$.
\end{lem}
\par
The dual problem, on continuous functions, corresponding to $(P)$ is the following
\begin{flalign}\nonumber
  & &  \inf_{\Xi}&\phantom{3} \ip{\lambda_x\otimes \lambda_\theta,w}          && (D) \nonumber \\
  & &  \text{st.}&\phantom{3}\mathcal L_{\tilde f} v(t,x,\theta)\le 0         && \forall (t,x,\theta)\in \mathcal T\times X\times\Theta\\
  & &  &\phantom{3} w(x,\theta) \ge 0                                         && \forall (x,\theta)\in X\times\Theta\\
  & &  &\phantom{3} w(x,\theta) - v(0,x,\theta) - 1 \ge 0                     && \forall (x,\theta)\in X\times\Theta\\
  & & & \phantom{3} v(T,x,\theta)\ge 0                                        && \forall (x,\theta)\in X_T\times \Theta
\end{flalign}
where $\Xi := (v,w)\in \mathcal C^1(\mathcal T\times X\times \Theta)\times \mathcal C(X\times \Theta)$. The solution to $(D)$ has an interesting interpretation: $v$ is similar to a Lyapunov function for the system, and $w$ resembles an indicator function on $\spt(\mu_0)$. Moreover:
\begin{lem}
  There is no duality gap between problems $(P)$ and $(D)$.
\end{lem}
\begin{lem}
  Given the pair of functions $(v^*,w^*)$ which is the optimal solution to $(D)$, the 1-super-level set of $w^*$ contains $\spt(\mu_0)$.
\end{lem}
The following salient result on the form of $w$ is a critical result that we will employ to estimate $X_0$ as defined in Defn.~\ref{defn:brs}.
\begin{thm}[henrion, thm 3]
\label{thm:indicator}
 There is a sequence of feasible points to $(D)$ whose $w$ component converges uniformly in the $L^1$ norm to the indicator function on $\spt(\mu_0)$.
\end{thm}
The immediate consequence of the above theorem is that we can assume that $w$ evaluates to one on $\spt(\mu_0)$ and zero elsewhere. Now, relating the definition of $\Gamma$ in Eqn.~(\ref{eq:Gamma}) and this feature of $w^*$, the $w$ component of the optimal solution of $(D)$, one arrives at the following result that provides a means to compute the $\alpha$-confidence time limited reachable set, $X_0$.
\begin{lem}
Suppose $(v^*,w^*)$ is an optimal solution of $(D)$. The $\alpha$-level backwards reachable of the set $X_T$ under the dynamics in Eqn.~(\ref{eq:aug_system}) and parametric uncertainty with distribution $\mu_\theta$ is given by the following set
\begin{align}
X_0^\alpha:=\bigg\{x\,\big \mid \int_\Theta w^*(x,\theta)\,d\mu_\theta\ge \alpha \bigg\}
\end{align}
\label{lem:confidence}
\end{lem}
\begin{proof}
%There exists a sequence $w_k$ of feasible $w$ in $(D)$ that converges to the indicator function $I_{\Gamma(x)}(x,\theta)$ in the $L^1$ norm (REFERENCE H-K PAPER). Therefore, the optimal solution $w^*$ is $I_{\Gamma(x)}(x,\theta)$. So, for any $x$,
%\begin{align}
%\int_\Theta w^*(x,\theta)\,d\mu_\theta &= \int_{\Gamma(x)} \mathds 1\,d\mu_\theta = \mu_\theta(\Gamma(x))
%\end{align}
Using the provided information, define the measure $\eta\in \mathcal M_+(X\times \Theta)$ as follows:
\begin{align}
  \eta(A\times B) = \int_{A\times B} w^*(x,\theta) \,d(\lambda_x\otimes \mu_\theta).
\end{align}
It should be noted that $\Gamma(x)$ as defined in Eqn.~(\ref{eq:Gamma}) is the support of the conditional distribution of $\theta$ given $x$ of $\eta$; $\spt(\eta(\cdot\mid x))$. This is true since for $w^*$ is an indicator function on $\spt(\mu_0)$, the set of all feasible pairs $(x,\theta)$.
In addition, by definition, $\lambda_x\otimes \mu_\theta \gg \eta$ and hence $\lambda_x\gg \pi^x_*\eta$, where $\pi^x_*$ is the push-forward of measure of $\eta$ under the projection operator \cite{lee2003smooth}. There exists $\phi(x)$ that is the Radon-Nikodym derivative between $\lambda_x$ and $\pi_*^{x}\eta$, the $x$-projection of $\eta$ such that
\begin{align}
  \pi^x_*\eta(A) =&\, \int_A \phi(x)\,d\lambda_x,\phantom{4}\forall A\subset X.
\end{align}
The function $\phi(x)$, for each $x$ evaluates to the probability that $x$ will reach $X_T$ given the distribution of uncertainty. To see this, observe that
\begin{align}
  \int_A \phi(x)\,d\lambda_x = &\,\int_A \int_\Theta w^*\,d\,\mu_\theta d\lambda_x,\\
  =&\, \int_A \int_{\Gamma(x)} w^*\,d\,\mu_\theta d\lambda_x,\\
  =&\, \int_A \int_{\Gamma(x)} 1\,d\,\mu_\theta d\lambda_x,
\end{align}
where we have used the fact that $w^*\ge 1,\, \forall(x,\theta)\in \spt(\mu_0)$ (from Thm.~\ref{thm:indicator}), that $\mu_\theta$ is a probability measure, and Defn.~\ref{defn:brs}. The statement of the Lemma now follows from Defn.~\ref{defn:brs}.
\end{proof}
Lemma~\ref{lem:confidence} provides a means to compute the $\alpha$-confidence $T$-time backwards reachable set; one just has to integrate the $w$ component of the optimal solution to $(D)$ with respect to the distribution of $\theta$ and identify level sets. Solving the infinite dimensional problem is nontrivial; in the following section, we employ Lasserre's hierarchy of relaxations to arrive at a sequence of outer approximations of $X_0^\alpha$.


==> sections/implementation.tex <==
\section{Numerical Implementation}
\label{sec:implementation}

\subsection{Generating Outer Approximations of $X_0^\alpha$}
\label{ssec:outer}
This section presents a method to use the outer approximations of $\spt(\mu_0)$ derived by solving $(D_d)$, to estimate $X_0^\alpha$ as defined in Defn.~\ref{defn:brs}. The method relies on discretizing the state space and computing the probability that each node in the mesh reach the target set $X_T$ at $t=T$, through Monte Carlo simulation.
%The second method poses an additional optimization problem over polynomial functions that computes a polynomial representation to the level sets of interest, whose solution can be outer-approximated by using semidefinite programming.

%\subsubsection{Direct Computation}
%\label{sssec:direct}
Given a $x_0$, to compute the probability of success, discretize the space of uncertainty, compute the spread of $w_d$ that solves $(D_d)$ with respect to $\theta$ as:
 \begin{align}
   \beta(x_0) :=\sum_{i=1}^N [\min\,\{1,w_d(x_0,\theta_i)\}]^k f_\theta(\theta_i)
   \label{eq:beta}
 \end{align}
 where $k\ge 1$, $\{\theta_i,\forall i\in \{1,\ldots,N\}\}$ is the set of discrete values of $\theta$, and $f_\theta(\theta)$ is the density (converted appropriately to a probability mass function) of $\mu_\theta$ with respect to $\lambda_\theta$. As the number of discretization points increases, this approach generates a convergent outer approximation of the $\alpha$-confidence BRS as shown in the following result.
\begin{lem}
\label{lem:outer:conv}
Given a desired confidence $\alpha$, let $w_d$ be the $w$ component of the optimal solution to $(D_d)$.
The direct computation method has the following properties as $k\rightarrow \infty$ and $N\rightarrow \infty$:
\begin{enumerate}[(a)]
  \item Given a $x_0\in X$
  \begin{align}
    \beta(x_0)\rightarrow \int\limits_{\{\theta\mid w_d(x_0,\theta)\ge 1\}} \min\,\{1,w_d(x_0,\theta)\}\,d\mu_\theta
    \label{eq:implementation:OA:m1:prop:convergence}
  \end{align}
  monotonically and is the estimated probability that the system, with initial condition $x_0$, arrives in $X_T$ at $t=T$.
  \item If $x_0 \in X_0^{\alpha}$, then $\beta(x_0) > \alpha$.
\end{enumerate}
\end{lem}
\begin{proof}[Proof~(Sketch)]
  The proof to part $(a)$ follows from the following observations: (i) the integrand on the right hand side of Eqn.~\eqref{eq:implementation:OA:m1:prop:convergence} is a polynomial; (ii) a density of $\mu_\theta$ wrt. $\lambda_\theta$ exists (Assumption~\ref{assump:mu_theta:abscont}); hence (iii) the right hand side of Eqn.~\eqref{eq:implementation:OA:m1:prop:convergence} is Riemann integrable. Finally, recognize that the definition of $\beta$ is the Riemann sum in question to complete the proof.
  \par
  To prove part $(b)$ recall that the 1-super-level-set of $w_d$ is an outer approximation of the the set of initial value pairs $(x,\theta)$ from which the solution trajectories arrive at $X_T\times \Theta$ at $t=T$. For all $x\in X$, let $\hat \Theta^x\subset \Theta$ be the smallest set (wrt. to $\lambda_\theta$) such that $\forall \theta\in \hat\Theta^x, w_d(x,\theta)\ge 1$. Let $w$ be the w-component of the solution to the corresponding infinite dimensional problem $(D)$, and define $\Theta_0^x:=\{\theta\in \Theta\mid w(x,\theta)\ge 1\}$. From Lemma~\ref{lem:implementation:outer}, $\Theta_0^x\subset \hat \Theta^x$; i.e. $\mu_\theta(\hat \Theta^x\backslash \Theta_0^x)\ge 0$. Now, from part \emph{(a)}, for each $x\in X$, $\beta(x)$ converges to $\mu_\theta(\hat \Theta^x)\ge \mu_\theta(\Theta_0^x)$. Thus, for each $x\in X^\alpha_0$, \mbox{$\beta(x)\ge \mu_\theta(\Theta_0^x)=\alpha$}.
\end{proof}
\begin{rem}
\label{rem:abs_const}
  It was assumed in Assumption~\ref{assump:mu_theta:abscont} that the distribution of the values of the uncertain parameters, $\mu_\theta$ satisfy $\mu_\theta \ll \lambda_\theta$. This assumption is not essential for the developments in Sections~\ref{sec:preliminaries} and \ref{sec:prob}. In fact, without this assumption, the definitions of $(P)$ and $(D)$ can be modified in the following way: (a) the right hand side of Eqn.~\ref{eq:primal:slack} becomes $\lambda_x\otimes \mu_\theta$; and (b) the objective function of $(D)$ becomes $\ip{\lambda_x\otimes \mu_\theta,w}$. In spite of the above changes, Lemmas~\ref{lem:primal:equiv}--\ref{lem:dual:level-set} and Theorems~\ref{thm:indicator} \& \ref{thm:uncertain_brs} remain unchanged.
  \par
  Assumption~\ref{assump:mu_theta:abscont} finds primary application in Section~\ref{ssec:outer} in the construction of the $\beta$ and the proof of Lemma~\ref{lem:implementation:outer} where the density of $\mu_\theta$ with respect to $\lambda_\theta$ is used in place of the measure $\mu_\theta$.
\end{rem}
%\subsubsection{Polynomial Optimization Approach}
%Consider the following optimization problem for a given value of $k$
%\begin{flalign}
%  &&\sup_{q,r} & \phantom{3}\ip{\lambda_x\otimes \mu_\theta,q} +\ip{\mu_\theta,r} && (PP)\\
%  &&\text{st. }&\phantom{3} 0\le q(x,\theta)\le 1                               && \forall (x,\theta)\in X\times \Theta\\
%  &&& \phantom{3} q(x,\theta) \le w(x,\theta)^k                                 && \forall (x,\theta)\in X\times \Theta\\
%  &&& \phantom{3}0\le r(x)\le \ip{\mu_\theta,q}                                 && \forall x\in X\\
%  &&& \phantom{3}r\in \R[x]\\
%  &&& \phantom{3}q\in \R[x,\theta]
%\end{flalign}
%The function $r$ is the function that traces the probability that every $x$ can reach $X_T$. The problem described in $(PP)$ is fundamentally similar to the direct computation method. Here, instead of employing spatial (parameter discretization), we seek to find a functional representation
%
%\ram{need an explanation as to why this works...and an explanation of where to look on how to approximate this reasonable...also can we have a lemma arguing that this is an outer approximation using the approximation to w?}
%\begin{lem}
%  ---
%\end{lem}

